A Proof of the MV Matching Algorithm

The Micali-Vazirani (MV) algorithm for maximum cardinality matching in general graphs, which was published in 1980 \cite{MV}, remains to this day the most efficient known algorithm for the problem. This paper gives the first complete and correct proof of this algorithm. Central to our proof are some purely graph-theoretic facts, capturing properties of minimum length alternating paths; these may be of independent interest. An attempt is made to render the algorithm easier to comprehend.

==> Equivalence.tex <==


\section{Equivalence of the Two Definitions of Blossom}
\label{sec.equivalence}

Below we establish equivalence of the two definitions of blossoms. 
Let us start by providing the definition of blossom as given in \cite{va.matching}; we will denote such a blossom of tenacity $t < l_m$ and 
base $b$ by $\bt^o$. Let $v$ be a vertex with $\t(v) \leq t$. 
We will say that an outer vertex $b$ is $\base_{> t} (v)$ if for some positive $k$, $\base^k (v) = b$, $\t(b) > t$,
and $\t(\base^{k-1} (v)) \leq t$. Then
\[ \bt^o = \{ v ~|~ \t(v) \leq t \ \mbox{and} \ \base_{>t} (v) = b \} .\]


\begin{theorem}
\label{prop}
The two definitions of blossom are equivalent, i.e., $\bt = \bt^o$.
\end{theorem}

\begin{proof}
Let $v \in \bt$. We will show that $v \in \bt^o$ by considering the following three cases. The set $S_{b, t}$ is defined in Definition \ref{def.blossom}.
\begin{enumerate}
\item
$v \in S_{b, t}$. In this case, $\t(v) = t$ and $\base(v) = b$, and therefore $\base_{>t} (v)) = b$. Hence $v \in \bt^o$.
\item
$v \in \CB_{b, t-2}$. In this case, $\t(v) < t$ and for some $k \geq 1$, $\base^k(v) = b$. Clearly, $\base^{k-1} (v) \in \CB_{b, t-2}$
and therefore $\base_{>t} (v) = b$. Hence $v \in \bt^o$.
\item
$v \in \CB_{u, t-2}$ and $u \in S_{b, t}$. In this case, $\t(v) < t$, $\t(u) = t$, $\base(u) = b$, and for some $k \geq 1$, $\base^k(v) = u$. Therefore,
$\base^{k+1} (v) = b$ and $\base_{>t} (v)) = b$. Hence $v \in \bt^o$.
\end{enumerate}

Next, let $v \in \bt^o$. Once again we will consider three cases to show that $v \in \bt$.
\begin{enumerate}
\item
$\t(v) = t$. In this case, $\base(v) = b$ and therefore $v \in S_{b, t}$. Hence $v \in \bt$.
\item
$\t(v) < t$, for some $k \geq 1$, $\base^k(v) = b$ and $\t(\base^{k-1} (v)) < t$. In this case, $v \in \CB_{b, t-2}$. Hence $v \in \bt$.
\item
$\t(v) < t$, for some $k \geq 1$, $\base^k(v) = b$ and $\t(\base^{k-1} (v)) = t$. Let $\base^{k-1} (v) = u$. Then,
$\t(u) = t$ and $\base(u) = b$. Therefore, $u \in S_{b, t}$ and $v \in \CB_{u, t-2}$. Hence $v \in \bt$.
\end{enumerate}
\end{proof}


==> talk.tex <==


Matching: A New Proof for an Ancient Algorithm



Vijay V. Vazirani

Georgia Tech




For all practical purposes, the Micali-Vazirani algorithm, discovered in 1980, is still the most efficient
known maximum matching algorithm (for very dense graphs, slight asymptotic improvement can be obtained using 
fast matrix multiplication). However, this has remained a "black box" result for the last 32 years. We hope 
to change this with the help of a recent paper giving a simpler proof and exposition of the algorithm:

http://arxiv.org/abs/1210.4594

In the interest of covering all the ideas, we will assume that the audience is familiar with basic notions
such as augmenting paths and bipartite matching algorithm.



